Measurement of the prompt $D^0$ nuclear modification factor in $p$Pb collisions at $\sqrt{s_\mathrm{NN}} = 8.16$ TeV

The production of prompt $D^0$ mesons in proton-lead collisions in the forward and backward configurations at a center-of-mass energy per nucleon pair of $\sqrt{s_\mathrm{NN}} = 8.16~\mathrm{TeV}$ is measured by the LHCb experiment. The nuclear modification factor of prompt $D^0$ mesons is determined as a function of the transverse momentum $p_\mathrm{T}$, and rapidity in the nucleon-nucleon center-of-mass frame $y^*$. In the forward rapidity region, significantly suppressed production with respect to $pp$ collisions is measured, which provides significant constraints of nuclear parton distributions and hadron production down to the very low Bjorken-$x$ region of $\sim 10^{-5}$. In the backward rapidity region, a suppression with a significance of 2.0 - 3.8 standard deviations compared to nPDF expectations is found in the kinematic region of $p_\mathrm{T}>6~\mathrm{GeV}/c$ and $-3.25<y^*<-2.5$, corresponding to $x\sim 0.01$.

==> acknowledgements.tex <==
\section*{Acknowledgements}
%
% These Acknowledgements valid from 3-May-2019
%
\noindent We express our gratitude to our colleagues in the CERN
accelerator departments for the excellent performance of the LHC. We
thank the technical and administrative staff at the LHCb
institutes.
We acknowledge support from CERN and from the national agencies:
CAPES, CNPq, FAPERJ and FINEP (Brazil); 
MOST and NSFC (China); 
CNRS/IN2P3 (France); 
BMBF, DFG and MPG (Germany); 
INFN (Italy); 
NWO (Netherlands); 
MNiSW and NCN (Poland); 
MEN/IFA (Romania); 
%MSHE (Russia); 
MICINN (Spain); 
SNSF and SER (Switzerland); 
NASU (Ukraine); 
STFC (United Kingdom); 
DOE NP and NSF (USA).
We acknowledge the computing resources that are provided by CERN, IN2P3
(France), KIT and DESY (Germany), INFN (Italy), SURF (Netherlands),
PIC (Spain), GridPP (United Kingdom), 
%RRCKI and Yandex LLC (Russia), 
CSCS (Switzerland), IFIN-HH (Romania), CBPF (Brazil),
Polish WLCG  (Poland) and NERSC (USA).
We are indebted to the communities behind the multiple open-source
software packages on which we depend.
Individual groups or members have received support from
ARC and ARDC (Australia);
Minciencias (Colombia);
AvH Foundation (Germany);
EPLANET, Marie Sk\l{}odowska-Curie Actions and ERC (European Union);
A*MIDEX, ANR, IPhU and Labex P2IO, and R\'{e}gion Auvergne-Rh\^{o}ne-Alpes (France);
Key Research Program of Frontier Sciences of CAS, CAS PIFI, CAS CCEPP, 
Fundamental Research Funds for the Central Universities, 
and Sci. \& Tech. Program of Guangzhou (China);
%Key Research Program of Frontier Sciences of CAS, CAS PIFI,
%Thousand Talents Program, and Sci. \& Tech. Program of Guangzhou (China);
%RFBR, RSF and Yandex LLC (Russia);
GVA, XuntaGal, GENCAT and Prog. Atracci\'on Talento, CM (Spain);
SRC (Sweden);
the Leverhulme Trust, the Royal Society
 and UKRI (United Kingdom).


